Shadow and Light: Digitally Reconstructed Radiographs for Disease Classification

In this paper, we introduce DRR-RATE, a large-scale synthetic chest X-ray dataset derived from the recently released CT-RATE dataset. DRR-RATE comprises of 50,188 frontal Digitally Reconstructed Radiographs (DRRs) from 21,304 unique patients. Each image is paired with a corresponding radiology text report and binary labels for 18 pathology classes. Given the controllable nature of DRR generation, it facilitates the inclusion of lateral view images and images from any desired viewing position. This opens up avenues for research into new and novel multimodal applications involving paired CT, X-ray images from various views, text, and binary labels. We demonstrate the applicability of DRR-RATE alongside existing large-scale chest X-ray resources, notably the CheXpert dataset and CheXnet model. Experiments demonstrate that CheXnet, when trained and tested on the DRR-RATE dataset, achieves sufficient to high AUC scores for the six common pathologies cited in common literature: Atelectasis, Cardiomegaly, Consolidation, Lung Lesion, Lung Opacity, and Pleural Effusion. Additionally, CheXnet trained on the CheXpert dataset can accurately identify several pathologies, even when operating out of distribution. This confirms that the generated DRR images effectively capture the essential pathology features from CT images. The dataset and labels are publicly accessible at https://huggingface.co/datasets/farrell236/DRR-RATE.

==> misc/notes.tex <==
Certainly! The Siddon-Jacobs ray tracing algorithm is known for its efficiency in calculating the path of rays through a voxel grid in medical imaging applications like CT scans. Here's a basic representation of the key equation used in the Siddon-Jacobs ray tracing algorithm:

Let's denote:
- \( \mathbf{p}_0 \) as the source point of the ray in 3D space.
- \( \mathbf{p}_1 \) as the endpoint of the ray on the detector.
- \( \mathbf{d} = \mathbf{p}_1 - \mathbf{p}_0 \) as the direction vector of the ray.
- \( t \) as the parameter that scales the direction vector.

The parametric equation of the ray can be expressed as:
\[ \mathbf{r}(t) = \mathbf{p}_0 + t \mathbf{d} \]

The ray intersects the voxel grid at discrete points, and the algorithm calculates these intersections along the ray path. The essential part of the algorithm involves finding \( t \) values where the ray crosses the planes defining the voxels in the grid. For a voxel grid defined by planes perpendicular to the \( x \), \( y \), and \( z \)-axes at regular intervals, the intersection points \( t_x \), \( t_y \), and \( t_z \) are calculated as follows:

\[ t_x(i) = \frac{x_i - x_0}{d_x}, \quad t_y(j) = \frac{y_j - y_0}{d_y}, \quad t_z(k) = \frac{z_k - z_0}{d_z} \]

where:
- \( (x_i, y_j, z_k) \) are the coordinates of the voxel boundaries,
- \( (x_0, y_0, z_0) \) are the components of \( \mathbf{p}_0 \),
- \( (d_x, d_y, d_z) \) are the components of \( \mathbf{d} \).

The algorithm then iterates through the sorted list of \( t \)-values to accumulate the voxel contributions along the ray, typically involving some form of interpolation or accumulation based on the material properties or density of the voxels.

This is a simplified version of the algorithm, as the actual implementation may involve optimizations and additional steps to handle various edge cases and efficiency considerations.


---

In the equations you've provided, several variables are involved in the computation of intersection points of a ray with the planes defining the voxels in a volume. Here's an explanation of each variable:

1. **\( t_x(i) \), \( t_y(i) \), \( t_z(i) \)**: These are the values representing the parameter \( t \) at which the ray intersects the planes corresponding to the \( x \), \( y \), and \( z \)-axes at the \( i \)-th interval. Each \( t \) value corresponds to a particular point along the ray where it crosses the planes defining the voxel boundaries.

2. **\( b_x \), \( b_y \), \( b_z \)**: These represent the base coordinates of the voxel grid along the \( x \), \( y \), and \( z \) axes, respectively. Essentially, these are the coordinates of the origin of the grid or the starting point of the voxel grid along each axis.

3. **\( \Delta\mathbf{X} \), \( \Delta\mathbf{Y} \), \( \Delta\mathbf{Z} \)**: These denote the intervals or the distance between consecutive planes along the \( x \), \( y \), and \( z \) axes. These are constants that define the size of each voxel in the respective dimensions.

4. **\( \mathbf{s}_x \), \( \mathbf{s}_y \), \( \mathbf{s}_z \)**: These are the \( x \), \( y \), and \( z \) components of the starting point \( \mathbf{s} \) of the ray. It is the point from which the ray originates.

5. **\( \mathbf{p}_x \), \( \mathbf{p}_y \), \( \mathbf{p}_z \)**: These are the \( x \), \( y \), and \( z \) components of a point \( \mathbf{p} \) on the ray, different from \( \mathbf{s} \). The vector from \( \mathbf{s} \) to \( \mathbf{p} \) defines the direction of the ray.

6. **\( i \)**: This is an index variable that increments to calculate each intersection point along a particular axis. For example, \( i \) can range from 0 to \( M \), where \( M \) is the number of intervals the ray crosses along that axis.

The formula for each \( t \)-value effectively computes where along the ray (parameterized by \( t \)) it intersects with each plane of the grid. The numerator calculates the difference between the plane's position and the ray's starting point along the axis, adjusted by \( i \) intervals of size \( \Delta \). The denominator computes the component of the ray's direction along that axis, indicating how quickly the ray moves along the axis as \( t \) increases. This setup is fundamental in ray tracing within voxel grids as used in medical imaging, simulation, and other computational geometry applications.
